Recycling Randomness with Structure for Sublinear time Kernel Expansions

We propose a scheme for recycling Gaussian random vectors into structured matrices to approximate various kernel functions in sublinear time via random embeddings. Our framework includes the Fastfood construction as a special case, but also extends to Circulant, Toeplitz and Hankel matrices, and the broader family of structured matrices that are characterized by the concept of low-displacement rank. We introduce notions of coherence and graph-theoretic structural constants that control the approximation quality, and prove unbiasedness and low-variance properties of random feature maps that arise within our framework. For the case of low-displacement matrices, we show how the degree of structure and randomness can be controlled to reduce statistical variance at the cost of increased computation and storage requirements. Empirical results strongly support our theory and justify the use of a broader family of structured matrices for scaling up kernel methods using random features.

==> introduction__1_.tex <==
Consider a $k$-dimensional feature map of the form,
\begin{equation}
\Psi(\vv{x}) = \frac{1}{\sqrt{n}} s(\vv{M} \vv{x}) \label{eq:featuremap}
\end{equation} where the input data vector $\vv{x}$ is drawn from $\reals^n$;  $s(\cdot)$ denotes a real-valued or complex-valued pointwise non-linearity (activation function); and $\vv{M}$ is an $k\times n$ Gaussian random matrix. It is well known that  as a function of a pair of data vectors,  the Euclidean inner product $\Psi(\vv{x})^T \Psi(\vv{z})$\footnote{In the complex case, $\Psi(\vv{x})^T$ denotes conjugate transpose.}, converges to a positive definite kernel function $k(\vv{x}, \vv{z})$  depending on the choice of the scalar nonlinearity, as $k\to\infty$. For example, the complex exponential nonlinearity $s(x) = e^{-i \frac{x}{\sigma}}$ corresponds to the Gaussian kernel~\cite{RahimiRecht}, while the rectified linear function (ReLU), $s(x) = \max(x, 0)$, leads to the Arc-cosine kernel~\cite{cho}.

In recent years, such random feature maps have been used to dramatically accelerate the training time and inference speed of kernel methods~\cite{KernelsBook, WahbaBook} across a variety of statistical modeling problems~\cite{RahimiRecht, LeSong} and applications~\cite{TIMIT, VedaldiZisserman2012}. Standard linear techniques applied to random nonlinear embeddings of the data are equivalent to learning with approximate kernels. To quantify the benefits, consider solving a kernel ridge regression task given $l$ training examples. With traditional kernel methods, dense linear algebra operations on the Gram matrix associated with the exact kernel function imply that the training complexity grows as $O(l^3 + l^2n)$ and the time to make a prediction on a test sample grows as $O(ln)$. By contrast, random feature approximations reduce training complexity to $O(l k^2 + lkn)$ and test speed to $O(kn)$. This is a major win on big datasets where $l$ is very large, provided that a small value of $k$ can provide a good approximation to the kernel function. 

In practice, though, the optimal value of $k$ is often large, albeit still much smaller than $l$. For example, in a speech recognition application~\cite{TIMIT} involving around two million training examples, it has been reported that of the order of a hundred thousand random features are required to match state of the art deep neural network models. In such settings, the time to construct the random feature map is dominated by matrix multiplication against the dense Gaussian random matrix, which becomes the new computational bottleneck. To alleviate this bottleneck,~\cite{LSS13} introduce the ``Fastfood" approach where Gaussian random matrices are replaced by Hadamard matrices combined with diagonal matrices with Gaussian distributed diagonal entries. It was shown in~\cite{LSS13} that for the specific case of the complex exponential nonlinearity, the Fastfood feature maps continue to provide unbiased estimates for the Gaussian kernel function, at the expense of additional statistical variance, but with the computational benefit of reducing the feature map construction time from $O(k n)$ to $O(k \log~n)$ by using the Fast Walsh-Hadamard transform for matrix multiplication.  The Fastfood construction for kernel approximations is akin to the use of structured matrices - in lieu of Gaussian random matrices - in Fast Johnson-Lindenstrauss transform (FJLT)~\cite{FJLT} for dimensionality reduction, fast compressed sensing~\cite{ToeplitzCS,CirculantCS}, and randomized numerical linear algebra techniques~\cite{HMT,Mahoney}

Our contributions in this paper are as follows:
\begin{compactitem}
\item We propose and analyze a new framework to define a broad family of structured matrices for fast 
feature map construction, which covers Fastfood features as a special case. Specifically, starting with 
a budget of randomness $t$, we show how a Gaussian vector $\vv{g}\in \reals^t$ can be recycled to create various classes of structured matrices.
\end{compactitem}

In section 2, we start with a brisk overview of 

\section{Background and Preliminaries}

\subsection{Random Embeddings, Nonlinearities and Kernels}

Random feature maps may be viewed as arising from Monte-Carlo approximations to integral representations of kernel functions. The original construction by ~\citet{RahimiRecht} was motivated by a classical result that characterizes the class of shift-invariant positive definite functions.

\begin{theorem}[Bochner's Theorem~\cite{bochner1933}] A continuous shift-invariant kernel
function $k(\x,\z)\equiv \phi(\x-\z)$ on $\reals^n$ is positive definite if and
only if it is the Fourier transform of a unique finite non-negative measure on
$\reals^n$.
That is, for any $\x,\z \in \reals^d $,
\begin{equation}
k(\x,\z) = \int_{\reals^n} e^{-i (\x-\z)^T\vv{w}} p(\w) d\w =
\Expectation_{\vv{w}\sim p}[ e^{-i (\x-\z)^T\vv{w}}]~.\nonumber\label{eq:bochner}
\end{equation}
\end{theorem} \label{thm:bochner_R_d}
Without loss of generality, the non-negative measure above can be assumed to be 
a probability measure with the associated density $p$. Bochner's theorem
establishes one-to-one correspondence between shift-invariant kernel functions
and probability densities on $\reals^n$, via the Fourier transform.  A Monte Carlo approximation to the integral above leads to the following,
\begin{equation}
k(\x, \z) \approx \frac{1}{k}\sum_{j=1}^k e^{-i \x^T \w_j} e^{i \z^T \w_j} =
\Psi(\x)^T \Psi(\z) 
\end{equation} where the feature map $\Psi(\x)$ has the form given in Eqn.~\ref{eq:featuremap},  with rows of $\vv{M}$ drawn from the density $p$.  For the Gaussian kernel with bandwidth $\sigma$, $k(\vv{x}, \vv{z}) = e^{\frac{-\|\vv{x} - \vv{z}\|}{2\sigma^2}}$, the associated density $p$ is also Gaussian, with $\sigma^{-2}$ times the identity as the covariance matrix. 
Equivalently, entries of $\vv{M}$ may be drawn i.i.d from a standard Gaussian distribution, if the complex exponential  $s(x) = e^{i \frac{x}{\sigma}}$ is used as the scalar nonlinearity. 

While studying synergies between kernel methods and deep learning~\cite{cho} introduce $b^{th}$-order {\it arc-cosine} kernels via the following integral representation:
$$
k_{b}(\vv{x}, \vv{z}) = \int_{\reals^d} i(\vv{w}^T \vv{x})  i(\vv{w}^T \vv{z}) (\vv{w}^T\vv{x})^b (\vv{w}^T \vv{z})^b \ p(\w) d\w 
$$ 
where $i(\cdot)$ is the step function, i.e.  $i(x) = 1$ if $x>0$ and $0$ otherwise; and the density $p$ is chosen to be standard Gaussian. 
These kernels evaluate inner products in the  representation induced by a infinitely wide single  hidden layer neural network with random 
Gaussian weights: for $b=0$, the activation function is hard thresholding, while $=1$ corresponds to using rectified linear units (ReLU). 
These kernels admit closed form expressions, in terms of the angle $\theta = cos^{-1} (\frac{\vv{x}^T\vv{z}}{\|\vv{x}\|_2\|\vv{z}\|_2})$ between $\vv{x}$ and $\vv{z}$:
\begin{eqnarray}
k_0(\vv{x}, \vv{z}) &=& 1 - \frac{\theta}{\pi}\label{eq:stepkernel}\\  
k_1(\vv{x}, \vv{z}) &=&  \frac{\|\vv{x}\|_2 \|\vv{z}\|_2}{\pi} [sin(\theta) + (\pi - \theta) cos(\theta)] \label{eq:relukernel}
\end{eqnarray} where $\| \cdot\|_2$ denotes $l_2$ norm. Therefore, feature maps of the form in Eqn.~\ref{eq:featuremap} with hard-thresholding ($s(x) = i(x)$) correspond to the angular similarity kernel in Eqn.~\ref{eq:stepkernel}, while ReLU activation $s(x) = max(x, 0)$ leads to the trigonometric kernel in Eqn.~\ref{eq:relukernel}.

\subsection{Structured Matrices}

\begin{figure*}[t]
\begin{minipage}{.3\linewidth}
~~~~~~~~~~~~~~~~(i) \textit{f-Circulant}
\begin{scriptsize}
\begin{eqnarray}
\left[\begin{array}{cccc} 
{\bf \color{red}{g_0}} & f {\bf g_{n-1}} & \ldots & f {\bf \color{blue} g_1}\\
{\bf \color{blue} g_1}& {\bf \color{red} g_0} & \ldots & \vdots\\
\vdots & \vdots & \vdots & f{\bf g_{n-1}} \\
{\bf g_{n-1}} & \ldots & {\bf \color{blue} g_1} & {\bf \color{red}g_0}
 \end{array}
 \right] \nonumber
\end{eqnarray}
\end{scriptsize}
\end{minipage}\hspace{-0.75cm}
\begin{minipage}{.3\linewidth}
~~~~~~~~~~~~~~~~(ii) \textit{Toeplitz}
\begin{scriptsize}
\begin{eqnarray}
\left[\begin{array}{cccc} 
{\bf \color{red}{t_0}} & {\bf \color{green} t_{-1}} & \ldots & {\bf \color{cyan}{t_{-(n-1)}}}\\
{\bf \color{blue} t_1}& {\bf \color{red} t_0} & \ldots & \vdots\\
\vdots & \vdots & \vdots & {\bf \color{green} t_{-1}} \\
{\bf t_{n-1}} & \ldots & {\bf \color{blue} t_1} & {\bf \color{red}t_0}
 \end{array}
 \right] \nonumber
\end{eqnarray}
\end{scriptsize}
\end{minipage}\hspace{-0.75cm}
\begin{minipage}{.5\linewidth}
~~~~~~~~~~~~~~~~(iii) \textit{Displacement rank r}
\begin{scriptsize}

\begin{eqnarray}
\sum_{i=1}^r \left[\begin{array}{cccc} 
{\bf \color{red}{g^i_0}} & {\bf g^i_{n-1}} & \ldots & {\bf \color{blue} g^i_1}\\
{\bf \color{blue} g^i_1}& {\bf \color{red} g^i_0} & \ldots & \vdots\\
\vdots & \vdots & \vdots & {\bf g^i_{n-1}} \\
{\bf g^i_{n-1}} & \ldots & {\bf \color{blue} g^i_1} & {\bf \color{red}g^i_0}
 \end{array}
 \right] 
\left[\begin{array}{cccc} 
{\bf \color{red}{h^i_0}} & -{\bf h^i_{n-1}} & \ldots & -{\bf \color{blue} h^i_1}\\
{\bf \color{blue} h^i_1}& {\bf \color{red} h^i_0} & \ldots & \vdots\\
\vdots & \vdots & \vdots & -{\bf h^i_{n-1}} \\
{\bf h^i_{n-1}} & \ldots & {\bf \color{blue} h^i_1} & {\bf \color{red}h^i_0}
 \end{array}
 \right] 
 \nonumber
\end{eqnarray}
\end{scriptsize}
\end{minipage}\\
\caption{Structured Matrices}\label{fig:structured}
\end{figure*}


A $m\times n$ matrix is called a structured matrix is it satisfies the following two properties: (1) it has much fewer degrees of freedom than 
$mn$ independent entries, and hence can be implicitly stored more efficiently than general matrices, and (2) the structure in the matrix can 
be exploited for fast linear algebra operations such as fast matrix-vector multiplication, factorizations and solution to linear systems.  
Examples include the Discrete Fourier Transform matrix (DFT) and the Discrete Cosine Transform matrix (DCT).  Here, we give other examples particularly relevant to this paper. 

{\bf Hadamard Matrices:} These matrices are defined for $m = n = 2^k$ recursively as follows:
\begin{equation}
\vv{H}_0 = 1,~~~~~~~~~~~\vv{H}_k = \frac{1}{\sqrt{2}} \left(\begin{array}{cc} \vv{H}_{k-1} & \vv{H}_{k-1}\\\vv{H}_{k-1} & -\vv{H}_{k-1} \end{array}\right)
\end{equation} Note that $\frac{1}{\sqrt{n}}\vv{H}$ is an orthonormal matrix. 
Hadamard matrices support $O(n~\log n)$ matrix-vector multiplication time via the Fast Hadamard transform, a variant of FFT. 

\def\krylov{\textrm{krylov}}
{\bf Circulant Matrices}: These matrices are intimately associated with circular  
convolutions and have been used for fast compressed sensing in~\cite{CirculantCS}. 
A $n\times n$ Circulant matrix is completely determined by  its first column/row, i.e., $n$ parameters. Each column/row of a Circulant 
matrix is generated by cyclically down/right-shifting the previous column/row. For righ-shifting one can define a Circulant matrix from $\mathbb{R}^{m \times n}$
for $m \leq n$ by taking first $m$ rows of the matrix described above.
An elementary matrix that implements a basic {\it downward shift-and-scale} transformation involving a scalar $f$ is called an $f$-unit-Circulant matrix, 
and is given below.

\begin{definition}[$f$-unit-Circulant Matrix] 
For a real-valued scalar $f$, the $(n\times n)$ f-unit-Circulant matrix, denoted by $\vv{Z}_f$, is defined as follows,
\begin{eqnarray}
\vv{Z}_f = \left[ \begin{array}{cc} 0_{1\times (n-1)} & {\color{red}f}\\ \vv{I}_{n-1} & 0_{(n-1)\times 1}\end{array}\right]\nonumber
\label{def:unitcirc}
\end{eqnarray}
\end{definition} where the notation $\vv{I}_n$  denotes a $n\times n$ identity matrix. 
The matrix-vector product $\vv{Z}_f \vv{v}$ shifts the elements of the column vector $\vv{v}$ ``downwards", scales by $f$ and brings the last element $v_n$ to the ``top", resulting in  $[{\color{red} f} v_n, v_1, \ldots v_{n-1}]^T$.  Define the matrix 
\krylov$(\vv{A}, \vv{v})$ by:
\begin{equation}
\krylov(\vv{A}, \vv{v}) = [\vv{v}~~\vv{A}\vv{v}~~\vv{A}^2 \vv{v} \ldots \vv{A}^{n-1} \vv{v}]\label{def:krylov}
\end{equation} 
Then it is easy to see that a Circulant matrix whose first column is $\vv{g}$ is simply $\krylov(\vv{Z}_1, \vv{g})$.  
We use the notation $\vv{Z}_1[\vv{g}]$ for a Circulant matrix. For $f=-1$, the matrix $\krylov(\vv{Z}_{-1}, \vv{g})$ is called skew-Circulant. For a general scalar $f$, the structure of $\vv{Z}_f[\vv{v}] = \krylov(\vv{Z}_{f}, \vv{g})$ referred to as an $f$-Circulant matrix is shown in Figure~\ref{fig:structured} (i). 
The class of $f$-circulant matrices admit $O(n~\log~n)$ matrix-vector multiplication as they are diagonalized by the DFT matrix~\cite{Pan}.
\iffalse
:
\begin{theorem}[Diagonalization of $f$-circulant matrices] 
For any $f\neq 0$,  let $${\bf f} = [1, f^\frac{1}{d}, f^\frac{2}{d}, \ldots f^{\frac{d-1}{d}}]^T \in \mathbb{C}^d,~~\textrm{and}~~\vv{D}_{\vv{f}} = diag(\vv{f})$$ and let $\Omega_d$ denote the matrix of the Fast Fourier Transform, i.e., $[\Omega_d]_{ij} = {\omega_d}^{ij}$ where $\omega_d = \exp{\left(\frac{i 2\pi}{d}\right)}$ denotes the $d$-th root of unity. Then, 
\begin{equation}
\vv{Z}_f[\vv{v}] = \vv{D}_{\vv{f}}^{-1}~\Omega_d^{-1}~diag(\Omega_d (\vv{f} \circ\vv{v})) \Omega_d \vv{D}_{\vv{f}}
\end{equation}
\end{theorem}\label{thm:f_circulant_diagonalization}
\fi

{\bf Toeplitz and Hankel Matrices:} These matrices implement discrete linear convolution and arise naturally in dynamical systems and time series analysis. Toeplitz matrices are characterized by constant diagonals (Fig~\ref{fig:structured}(ii)), while closely related Hankel matrices have constant anti-diagonals. Matrix-vector multiplication for these matrices taken from $\mathbb{R}^{m \times n}$ can be reduced to $O(n~\log~m)$ Circulant matrix-vector multiplication. For detailed properties of Circulant and Toeplitz matrices, we point the reader to~\cite{GrayCirculantToeplitz}

{\bf Structured Matrices with Low-displacement Rank}: The notion of displacement operators and displacement rank~\cite{Golub, Pan, KKM79} can be used to broadly generalize various classes of structured matrices.  For example, under the action of the {\it Sylvester displacement operator} defined as $$L[\vv{T}] = \vv{Z}_1 \vv{T} - \vv{T} \vv{Z}_{-1},$$  every Toeplitz matrix can be transformed into a matrix of rank at most $2$ using shift and scale operations. For a given displacement rank parameter $r$, the class of matrices for which the rank of $L[\vv{T}]$ is at most $r$ is called {\it Toeplitz-like}, and in fact admits a closed-form parameterization:

\begin{theorem}[Parameterization of Toeplitz-like matrices with displacement rank r] (Pan, 2003):  If a $n\times n$ matrix $\vv{T}$ satisfies $rank(\vv{Z}_1 \vv{T} - \vv{T} \vv{Z}_{-1}) \leq r$  then $\vv{T}$ can be written as,
\begin{equation}
\vv{T} = \sum_{i=1}^r \vv{Z}_1[\vv{g}^i] \vv{Z}_{-1}[\vv{h}^i] \label{eq:circ_skewcirc}
\end{equation}
\end{theorem}
Note that the notation $\vv{Z}_f$ refers to $f$-unit-Circulant matrix (Definition~\ref{def:unitcirc}) while $\vv{Z}_f[\vv{g}] = \krylov(\vv{Z}_f, \vv{g})$ (see Eqn.~\ref{def:krylov}).
Instead of $T \in \mathbb{R}^{n \times n}$ defined above one can also take its first $m$ rows ending up with a structured matrix from $\mathbb{R}^{m \times n}$.
This family of matrices expressible by Eqn.~\ref{eq:circ_skewcirc} for a suitable choice of vectors $\{\vv{g}^i, \vv{h}^i\}_{i=1}^r$,  is very rich, i.e., it covers (i) 
all Circulant and Skew-circulant matrices for $r=1$, (ii) all Toeplitz matrices and their inverses for $r=2$, (iii) Products, inverses, linear combinations of distinct 
Toeplitz matrices with increasing $r$, and (iv) all $n\times n$ matrices for $r=n$. 
Since Toeplitz-like matrices under the parameterization of Eqn.~\ref{eq:circ_skewcirc} 
are a sum of products between Circulant and Skew-circulant matrices, their fast FFT based matrix-vector multiplication is of order $O(nr log~m)$,
where $r$ is the displacement rank. Hence, $r$ provides a knob with which to control the storage requirements, 
computational constraints and statistical capacity of Toeplitz-like structured matrices. Recently such matrices were used in the context of 
learning mobile-friendly neural networks in~\cite{StructuredTransforms}. We note in passing that the displacement rank framework generalizes 
to other types of base structures (e.g. Vandermonde); see~\cite{Pan}.
 
%This displacement rank approach  unifies algorithms and complexity analysis for structured matrices~\cite{KKM79},~\cite{Pan},~\cite{KS95}. 

%\begin{compactitem}
%\item The complex exponential $s(x) = e^{-i \frac{x}{\sigma}}$ corresponds to the Gaussian kernel, $k(\vv{x}, \vv{z}) = e^{\frac{-\|\vv{x} - \vv{z}\|}{2\sigma^2}}$.
%\item 
%\end{compactitem}

%\begin{table}[h]
%\begin{center}
%{\small
%\begin{tabular}{cccc}
%Nonlinearity & $s(x)$ & Kernel & $k(\vv{x}, \vv{z})$\\
%\hline
%Complex-Exp. & $e^{-i x/\sigma}$  & Gaussian & $$\\
%ReLU & $\max(x, 0)$ & Arc-cosine & $\frac{\|x\|_2 \|z\|_2}{\pi} [sin(\theta) + (\pi - \theta) cos(\theta)]$\\
%Step & $1[x>0]$ & Angle	 & $(\pi - \theta)$\\
%\hline
%\end{tabular}
%}
%\end{center}
%\end{table}

\subsection{FastFood}
In the context of fast kernel approximations,~\cite{LSS13} introduce the Fastfood  technique where the matrix $\vv{M}$ in Eqn.~\ref{eq:featuremap} is parameterized by a 
product of diagonal and simple matrices as follows:
\begin{equation}
\vv{F} = \frac{1}{\sqrt{d}}\vv{S}\vv{H}\vv{G} \vv{P} \vv{H} \vv{B}.
\end{equation} Here, $\vv{S}, \vv{G}, \vv{B}$ are diagonal random matrices, $\vv{P}$ is a permutation matrix and $\vv{H}$ is the Walsh-Hadamard matrix.  
The $k\times n$ matrix $\vv{M}$ is obtained by vertically stacking $k/n$ independent copies of $\vv{F}$. Multiplication 
against such a matrix can be performed in time $O(k\log~n)$. The authors prove that (1) the Fastfood approximation is 
unbiased, (2) its variance is at most the variance of standard Gaussian random features with an additional $O(\frac{1}{k})$ 
term, and (3) for a given error probability $\delta$, the pointwise approximation error of a $n\times n$ block of Fastfood is 
at most $O(\sqrt{\log(n/\delta)})$ larger than that of standard Gaussian random features. However, note that the Fastfood analysis 
is limited to the Gaussian kernel and their variance bound uses properties of the complex exponential. The authors also conjecture 
that the Hadamard matrix $\vv{H}$ above, can be replaced by any matrix $\vv{T}$ such that $\vv{T}/\sqrt{n}$ is orthonormal, the 
maximum entry in $\vv{T}$ is small, and matrix-vector product against $\vv{T}$ can be computed in $O(n\log~n)$ time.
